Helix: Holistic Optimization for Accelerating Iterative Machine Learning

Machine learning workflow development is a process of trial-and-error: developers iterate on workflows by testing out small modifications until the desired accuracy is achieved. Unfortunately, existing machine learning systems focus narrowly on model training---a small fraction of the overall development time---and neglect to address iterative development. We propose Helix, a machine learning system that optimizes the execution across iterations---intelligently caching and reusing, or recomputing intermediates as appropriate. Helix captures a wide variety of application needs within its Scala DSL, with succinct syntax defining unified processes for data preprocessing, model specification, and learning. We demonstrate that the reuse problem can be cast as a Max-Flow problem, while the caching problem is NP-Hard. We develop effective lightweight heuristics for the latter. Empirical evaluation shows that Helix is not only able to handle a wide variety of use cases in one unified workflow but also much faster, providing run time reductions of up to 19x over state-of-the-art systems, such as DeepDive or KeystoneML, on four real-world applications in natural language processing, computer vision, social and natural sciences.

==> overview-survey.tex <==
%!TEX root=../dml.tex

%\begin{figure*}
%\centering
%\includegraphics[width= 0.27\paperwidth,height = 0.20\paperheight]  {figures/actionresult.png} 
%\includegraphics[width= 0.27\paperwidth,height = 0.20\paperheight]  {figures/actionresult2.png}   
%\includegraphics[width= 0.27\paperwidth,height = 0.20\paperheight]  {figures/actionresult3.png}     
%\caption{Proportion of variants of the ML workflow in different application areas.}
%\label{fig:actionresult}    
%\end{figure*}

%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{figures/domainConfBar}
%\caption{Paper topic domains by conference.
%\dorx{This isn't all that interesting. Can be removed/condensed.}}
%\label{fig:domBar}
%\end{figure}

\begin{figure*}[th]
\centering
\includegraphics[width=\textwidth]{figures/surveyResults.png}
\caption{(a) Paper count by domains for conference included in the literature survey. 
(b) Fraction of papers with each characteristic in each domain.
(c) The average DRP, L/I, and PPR iterations for each domain.
\dorx{The color scheme for (c) matches the color scheme in Figure~\ref{fig:wfEx}.}}
\label{fig:survey}
\end{figure*}

ML workflow development is anecdotally 
regarded to be highly iterative in nature, 
due to the unpredictable performance 
arising from data variability 
and model complexity~\cite{lin2013scaling,sumbaly2013big}.
However, to the best of our knowledge, 
no quantitative studies of iteration exist in the literature.
To remedy this, we conducted a small-scale 
survey of the applied ML literature,
trying to analyze the workflow variations 
corresponding to the results reported in each paper.
Note that since
authors report on only a small subset of iterations
necessary to produce the experimental results presented in the paper,
this survey captures only a limited view of the iterative process.
%; 2) authors often do not report the order in which the results are obtained.
%For example, we discovered that computer vision papers from CVPR conventionally 
%present only the final model parameters but not the tuning process.
Thus, our findings are merely a lower bound 
on the actual number of iterations.
Nevertheless, the survey provides valuable insights into common practices
for iterating on ML workflows.


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{figures/iterationDomainBar}
%\caption{Average Number of DPR, L/I, and PProc Iterations by Application Domain.\agp{These figures are eventually going to have to be cleaned up, made consistent, and with increased fonts so that it can be shrunk if need be. I dislike the color schemes (but that's the least of the issues), and the fact that some are horizontal while others vertical.}}
%\label{fig:iterCount}
%\end{figure}

We surveyed 105 papers randomly sampled 
from KDD~'16 Applied Data Science Track, ACL~'16, Nature~'16, and CVPR~'16,
spanning applications in social sciences (SocS), web applications (WWW), natural sciences (NS), natural language processing (NLP), and computer vision (CV).
\agp{I think you should describe what the inclusion criteria were.}
\dorx{``randomly sampled?''}
Paper topics were determined using the ACM Computing Classification System.
See Figure~\ref{fig:survey}(a) for paper counts by conference and topic.

For each paper, we recorded details about 
the datasets, feature engineering steps, 
ML models and optimization algorithms, 
and evaluation methods.
To approximate the number of DPR, L/I, and PPR iterations in each paper, we use the following estimators:
\begin{denselist}
\item DPR: the number of feature transformation methods (e.g., normalization);
\item L/I: $n_{ml} - 1$, where $n_{ml}$ is the number of ML algorithms (e.g., SVM), 
	optimization techniques (e.g., SGD) 
	and model tuning steps (e.g., regularization);
	%\footnote{We subtract 1 from this count to exclude the initial model from the iteration count.}.
\item PPR: $min(n_{metrics}, n_{ft})$, where $n_{metrics}$ is the number of metrics reported 
(counting closely related metrics, such as precision and recall, as one),
and $n_{ft}$ is the number of figures and/or tables containing evaluation results.
%We assume that each table/figure and 
%disparate metrics require their own PPR iteration
%and avoid overestimation by taking the minimum of the two counts.
\end{denselist}
\dorx{Here is a justification for all three estimators instead of individual ones.}
Assuming that at most one variable is changed between two iterations, 
these estimators are all lower bounds 
because they count only the distinct results
but not the transitions between them.
Treating each result as a node in a connected graph,
the number of edges is lower bounded by the number of nodes minus one.

\noindent Figure~\ref{fig:survey}(c) shows
the average number of each type of iteration 
for workflows by application domain. 
CV and NLP workflows have fewer DPR iterations, 
due to the fact that all surveyed papers 
study the same preprocessed and annotated datasets, 
in addition to the prevalence of deep neural networks (DNNs).
We discovered that by convention, 
CV papers report only the final model parameters 
and not the entire model tuning process, 
hence the below-average number of L/I iterations.
On the other hand, NS papers tend to report  
on a larger number of models (e.g., SVM, Random Forest)
since the applicability of a model class to the problem investigated
presents value to future researchers
(SVM is the most popular choice by a large margin).
Overall, the average (max) numbers of DPR, L/I, and 
PProc iterations are 1.3 (5), 1.5 (7), and 2.8 (6), respectively.
% , 
% which are greater than the topic-specific averages for CV and NLP
% but not SocS, NS, and WWW. \agp{Why is the previous bit important?}
We also find that the average number of iterations is four or more
across all domains, with WWW, SocS, and NS papers reporting
an average of $> 6$ iterations. 

In addition, we highlight four interesting characteristics 
discovered during our survey in Figure~\ref{fig:survey}(b). 
First, web applications and SocS are much more likely 
to incorporate \textit{multiple data sources} in creating an ML model.
Here, we focus on cases where a single model relies on multiple data sources,
not the case where models are evaluated on multiple datasets.
For web applications, this often entails joining log data with user profiles;
SocS often consider both the social network and auxiliary information such as geographic features.
Second, except in CV, \textit{most domains still rely upon 
features handcrafted by domain experts.} 
%such as the \textit{Residential Community Features} in Zhu et al.\cite{zhu2016days}.
%, despite the popular belief that such practices are antiquated 
%with the advent of deep neural networks (DNN)
%\footnote{Note that all surveyed papers are from 2016.}
%\agp{Why is this resident community feature so important? if important, describe what it is, else skip.}
Third, contrary to common belief, 
deep neural networks are not
ubiquitously adopted, especially in SocS and web applications,
due largely in part to limited data and computing resources availability, 
and to the lack of human interpretability of outputs.
Lastly, in addition to reporting aggregate metrics such as AUC,
authors often conduct fine-grained case studies on specific datapoints 
to elucidate the limitations of their approach.  
Almost every CV paper contains case studies since images readily lend themselves to visualization.
Furthermore, authors in natural sciences study specific high-impact features
to derive new scientific insights.

%\begin{figure}
%\centering
%\includegraphics[scale=0.55]{figures/funSurveyFacts}
%\caption{Notable Characteristics of ML Workflows by Domain.}
%\label{fig:funFact}
%\end{figure}

We use iteration trends presented in Figure~\ref{fig:survey}(c) 
to guide our empirical evaluations in Section~\ref{sec:experiments};
specific system design decisions are informed by 
insights presented in Figure~\ref{fig:survey}(b).

% common metrics?


%  ------ old version below -------
%\shit{Common ML folklore knowledge indicates that ML workflows are seldom ``perfect''
%on the first attempt and require significant iteration
%to improve accuracy~\cite{lin2013scaling,sumbaly2013big}.
%To confirm this, we surveyed papers
%from a variety of machine learning application areas to check for
%the presence of {\em workflow iterative actions}, involving some sort of
%user-instigated modification of one or more ML workflows presented in each paper.
%%We found that nearly every paper had some example of a {\em workflow action};
%%that is, a tweak to the data preparation, learning, or inference step(s) of a given workflow.
%Naturally, this survey has one major limitation ---
%authors often omit the exact number
%of iterations 
%\dorx{It's not just the number we're interested in. 
%We need to know what the iterations are.} 
%taken along the way to the reported findings.
%Nonetheless, it provides valuable insights into the kinds
%of ``knobs'' that are often used to tune ML workflows.}
%
%%While iterating on machine learning workflows is a widely adopted practice
%%in developing real-world applications~\cite{lin2013scaling, sumbaly2013big},
%%we are not aware of any evidence that 
%%quantitatively characterizes this iterative process.
%%\dorx{Rewrote the sentence above because I didn't find any reference to iteration in \cite{munson2012study}.}
%%To remedy this, we conducted a small scale survey of 
%%the applied ML literature across multiple fields
%%to catalog the frequency of various workflow modification actions.
%%Naturally, this survey has one major limitation ---
%%authors often omit reporting on a number
%%of iterations the taken to get to the reported findings.
%%Nevertheless, it provides valuable insights into the kinds
%%of ``knobs'' that are often used to tune ML workflows.
%
%\shit{\agpquote{We selected 5 application areas for machine learning, and one or more
%publication venues for each of them---Social Sciences (KDD), Natural Sciences (KDD, Nature), Computer Vision (KDD, CVPR), Natural Language Processing (KDD, ACL), and Web Mining (KDD) with 25, 37, 20, 37, and 12 papers
%from each area, respectively. The papers were all published in either 2015 or 2016.}{Maybe provide some details?}
%\agpquote{``Iteration actions'' present in the papers fell broadly into two categories:
%data preparation (DPR), or learning/inference (L/I).
%DPR actions include addition, deletion, or transformation of the raw data~\cite{kuhn2013data}, and L/I iteration actions
%include any tweak to the learning algorithm, including
%(but not limited to) adjustment of regularization or other hyperparameters,
% model selection, ablations of the core workflow, and other modifications for error analysis.}{You are just repeating 2.1.}
% \ \\
% \agp{Can we provide some examples of interesting insights? E.g. NLP requires more blah. Right now, feels like
% you cooked up numbers from thin air.}
%\frameme{Overall, we found that
%{\em nearly every paper exhibited some sort of iteration on at least one ML workflow}, with
%a roughly 50/50 split between adjustments to DPR and adjustments to L/I.}}
%\placeholder{We will release our survey's paper list, its associated code,
%and our detailed analysis of the results along with the rest of the \gs codebase upon this manuscript's
%acceptance for publication.}
%\smc{Placeholder sentence until we decide whether we want to put more detailed survey plots in appendex,
%techreport, or release with code.}
%
%\hidden{We manually classified each variant of the ML workflow described
%in each of these papers based on \dorx{rewrite the rest of this section from this point.} a transformation to either DPR or L/I, where DPR generally refers to the addition, deletion, or transformation of the training set data\cite{kuhn2013data} and L/I refers to any operation towards machine learning algorithm.
%% \dorx{Iterating on the DPR component involves ..., whereas iterating on L/I involves ... I don't know if you need this sentence if you're listing the actions in the next one.}
%Within
%DPR, we classified each variant into either 
%feature selection (select a subset of features), feature normalization (normalize independent variables of features into the range [0,1]), or feature transformation (apply a set of operators such as \{$+$, $-$, $*$\} on the original feature values\cite{sondhi2009feature}), and within L/I, we classified each variant into either
%a change of machine learning algorithm (i.e., switch the current ML model type, such as substituting SVM for logistic regression), 
%a change in tuning parameters (also known as model tuning which is adjusting the hyperparameters of the model training algorithms),
%or a change in model structure (e.g. adding L1/L2-regularization or adding an attention layer). 
%
%\topic{Quantitative Study Results} 
%To catalog the frequency of DPR and L/I, we judge each paper separately, where each variant within DPR and L/I was recorded. 
%The results are tabulated in Figure~\ref{fig:actionresult}(a) - (c), where the X axis is organized along different application areas, and the Y axis is the proportion of papers containing the corresponding ML workflow variant on the X.
%Figure~\ref{fig:actionresult}(a) is for the proportion of DPR and L/I in 5 application areas. Figure~\ref{fig:actionresult}(b) is for the proportion of the 3 primary DPR variants (feature selection, feature normalization and feature transformation) and Figure~\ref{fig:actionresult}(c) is for the proportion of the 3 primary L/I variants (ML algorithm change, model tuning and model structure change).
%% , where the X axis is organized along different application areas, and the Y axis is, the proportion of the number of papers in sampling papers containing the corresponding ML workflow variant on the X.
%
%
%Of all the papers we surveyed every single one of them contained some kind of iterative actions.
%As can be seen from the figure, variants of both DPR and L/I
%are often explored in applied machine learning papers;
%% specifically, more than 50\% of ML application papers displayed some variants on either DPR or L/I. 
%Similarly, we find that all three DPR variants,
%and all three L/I variants are common across all application areas.
%That said, there were some interesting special cases.
%For example, Figure~\ref{fig:actionresult}(a) shows that experts in Natural Sciences make more effort on Learning/Inference, which is different from experts in other application areas. This may because that experts in this application area are not quite familiar with ML. Therefore, when they try to optimize their ML workflow, they are not as confident with what is the right "general approach" and thus try different hyperparameters or just change their ML algorithm. 
%% By refering to Figure~\ref{fig:actionresult}(b), we notice that experts in Web Mining do more feature selection optimization than others. It is because that they 
%% Experts in Computer Vision make much more effort on feature transformation. It may be due to that a main problem in this area is how to interpret images and the problem convert to how to transform a image into better features when applying ML.
%% \dorx{break this into multiple sentences or condense. Also, you might want to give examples of feature transformations they do in CV because most readers would raise an eyebrow at the claim that a lot of feature transformation is done in CV.} 
%% Therefore, experts in this area use transformation processes to improve prediction accuracy. 
%Besides, we can find from Figure~\ref{fig:actionresult}(c) that experts in Natural Language Processing and Computer Vision have much more tendency to change model structure than others. It is because that experts in these areas use neural network to solve their problem frequently (more than 50\% of the sampling papers use neural network as one of the ML models) and thus they do more actions like add or remove a layer when adjusting the ML algorithm.}

% model structure change is the most frequent for experts in Natural Language Processing and Computer Vision when they tend to adjust their ML models, which 

% \dorx{Break into multiple sentences or condense. At this point I'm still puzzled by the result that CV people do a lot of feature transformations despite using NNs, which are supposed to reduce the need for feature engineering.}


% the tendency to pay more attention on transforming text data into appropriate data format in order to implement ML methods and improve prediction accuracy.







 % This may be caused by that experts in this application area have more tendency to make effort on how to build their ML model such as tuning the hyperparameters and changing the structure of model (shown in Figure~\ref{fig:actionresult}(c)).  For data preparation, they usually only use several sentences to explain how they select the features.


  % By referring to Figure~\ref{fig:actionresult}(b), it is shown that experts in Natural Language Processing make much more effort on feature transformation, which may be due to the tendency to pay more attention on transforming text data into appropriate data format in order to implement ML methods and improve prediction accuracy. 



  





% the variants in all application areas are on DPR and on L/I. 







% By referring to Figure~\ref{fig:actionresult}c), that condition is partly beacuse 




% \agp{plot has TOO small of a font. Needs to be much larger. It's Learning/Inference, 
% not Learning. "Detail in Blah" can be avoided. Just say "Data Preparation Breakdown", "Learning/Inference Breakdown" etc.}

% \agp{potentially delete everything below once gaps are filled in ==========}


% \todo{\dorxsubst{Stas}{Stats} work and need some comment}
% \dorx{What is an action in the context of this section?}
% As is mentioned above, ML workflows can be decomposed to data preparation and learning/inference. We regard these two components as two main actions in ML: Data Preparation and Learning. 
% \dorx{Two main categories of actions maybe. 
% They are not refinement actions themselves.}
% \dorxsubst{Data Preparation generally refers to}
% {Iterative refinements to the data preparation component may include} the addition, deletion, or transformation of the training \dorxout{set} data\cite{kuhn2013data}. 
% It contains feature selection, feature formats transformation, normalization etc. Learning contains actions of switching different types of model, modifying objective model structure, model tuning etc. 
% \dorx{Okay none of these terms mean much to someone who has little ML background. 
% Put them in the context of what has already been introduced.}

% Action information is what indicates the machine learning users' actions. 
% \dorxout{To refine the iteration,} we evaluate what experts in different research field tend to do in order to optimize their ML workflow by \dorxsubst{randomly selecting}{sampling} 120 papers from KDD 2016, ACL 2016 and Nature and extracting action information from them. According to the papers used, we divide the research field into 5 aspects: Social Sciences, Natural Sciences, Computer Vision, Natural Language Processing and Web Mining. The results are shown in Figure~\ref{fig:actionresult}.

% \dorx{What is the overall trend before you talk about individual subject areas.}
% \dorxsubst{According to}{As shown in} Figure~\ref{fig:actionresult}a), experts in Social Sciences, Computer Vision, Natural Language Processing and Web Mining make more effort on data preparation. However, Natural Sciences experts do more things on learning. For data preparation, Figure~\ref{fig:actionresult}b) shows that transforming feature formats is the most frequent action for experts in Computer Vision and Natural Language Processing and filter/select feature is the most frequent in other research field. For learning stage, Computer Vision and Natural Language Processing experts have a greater tendency to modify model structure, but experts in other research field make more effort on model tuning.
% \dorx{Okay can you say something about what contributes to this difference?}

% ML workflow iteration can be refined based on different tendency of different research field.


% \todo{add figures}
% We divided Learning/inference into two sub-category: Model Specification and Optimization. Any modification to the objective component of a machine learning model is a Model Specification action, such as switching the model, modifying objective model structure and model tuning. Optimization are actions that optimize the performance of the model on the basis of not changing the objective component of the model, such as adjusting batchsize of the neural network. Besides, changing the iteration number is also Optimization. 
% Result(figure) and comment?
% \todo{add .did add picture}
% \todo{outline}






==> overview-survey2.tex <==
%!TEX root=../dml.tex

%\begin{figure*}
%\centering
%\includegraphics[width= 0.27\paperwidth,height = 0.20\paperheight]  {figures/actionresult.png} 
%\includegraphics[width= 0.27\paperwidth,height = 0.20\paperheight]  {figures/actionresult2.png}   
%\includegraphics[width= 0.27\paperwidth,height = 0.20\paperheight]  {figures/actionresult3.png}     
%\caption{Proportion of variants of the ML workflow in different application areas.}
%\label{fig:actionresult}    
%\end{figure*}

%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{figures/domainConfBar}
%\caption{Paper topic domains by conference.
%\dorx{This isn't all that interesting. Can be removed/condensed.}}
%\label{fig:domBar}
%\end{figure}

%\begin{figure*}[th]
%\centering
%\includegraphics[width=\textwidth]{figures/surveyResults.png}
%\caption{(a) Paper count by domains for conference included in the literature survey. 
%(b) Fraction of papers with each characteristic in each domain.
%(c) The average DRP, L/I, and PPR iterations for each domain.
%\dorx{The color scheme for (c) matches the color scheme in Figure~\ref{fig:wfEx}.}}
%\label{fig:survey}
%\end{figure*}

ML workflow development is anecdotally 
regarded to be highly iterative~\cite{lin2013scaling,sumbaly2013big}.
However, 
there is limited quantitative evidence to 
characterize iteration in ML workflow development.
To this end, we analyzed a sample of applied ML papers. More details can be
found in Xin et al.~\cite{xin2018developers}; we provide a brief summary here.
We collected statistics from papers from
five application domains: 
computer vision (CV), natural language processing (NLP), web applications (WWW),
natural sciences (NS), and social sciences (SS).
The statistics collected pertain to 
the frequency of operations 
in the three workflow components introduced above.
While academic papers present 
only a partial view of the development process,
our survey nevertheless sheds light on common practices
for iteration.

% \begin{figure*}
% \begin{subfigure}{0.25\textwidth}
% \vspace{-60pt}
% \includegraphics[width=\linewidth]{figures/meanCountPOB.pdf}
% \includegraphics[width=\linewidth]{figures/funFacts.pdf}
% \end{subfigure}
% \includegraphics[width=0.33\textwidth]{figures/sys6.pdf}
% \includegraphics[width=0.33\textwidth]{figures/wf-lifecycle2.pdf}
% \end{figure*}

\begin{figure}
\begin{subfigure}{0.45\textwidth}
\centering
\caption{}
\vspace{-3pt}
\includegraphics[width=0.6\linewidth]{figures/meanCountPOB.pdf}
\label{fig:iterCount}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\centering
\vspace{4pt}
\caption{}
\vspace{-7pt}
\includegraphics[width=0.8\linewidth]{figures/funFacts.pdf}
\label{fig:funFacts}
\end{subfigure}
\vspace{5pt}
\caption{ \subref{fig:iterCount} The average DRP, L/I, and PPR iterations for each domain;
\subref{fig:funFacts} Fraction of papers with each characteristic by domain.}
\label{fig:survey}
\vspace{-15pt}
\end{figure}

Each iteration is categorized by the workflow components modified in that iteration,
e.g., an iteration in which the user changes learning parameters is an L/I iteration.
Figure~\ref{fig:iterCount} shows
the average number of DRP, L/I and PPR iterations 
for each application domain.
Overall, the average (max) numbers of DPR, L/I, and 
PProc iterations are 1.3 (4), 1.2 (5), and 2.6 (5), respectively.
The global average number of iterations is 5.1 across all domains\techreport{; 
SS and NS exceed the global average;
WWW is on par with the global average;
CV and NLP fall below the global average}.
CV workflows have fewer DPR iterations, 
due to the fact that all surveyed CV papers 
study the same preprocessed datasets, 
and often use deep neural networks (DNNs).
We found that by convention, 
CV and NLP papers report only the final model parameters 
and not the entire model tuning process, 
hence the below-average number of L/I iterations.
NS papers tend to report  
on a larger number of models (e.g., SVM, Random Forest)
since the applicability of a model class 
to the problem investigated
presents value to future researchers 
(SVM is the most popular choice by a large margin).

In addition, we highlight four interesting characteristics 
discovered during our survey in Figure~\ref{fig:funFacts}. 
First, WWW and SS are much more likely 
to incorporate \textit{multiple data sources} in creating an ML model.
\techreport{Here, we focus on cases where a single model relies on multiple data sources,
not the case where models are evaluated on multiple datasets.}
For WWW, this often entails joining log data with user profiles;
SS often considers both the social network 
and auxiliary information such as geographic features.
Second, except in CV, most domains still rely upon 
features handcrafted by domain experts. 
%such as the \textit{Residential Community Features} in Zhu et al.\cite{zhu2016days}.
%, despite the popular belief that such practices are antiquated 
%with the advent of deep neural networks (DNN)
%\footnote{Note that all surveyed papers are from 2016.}
%\agp{Why is this resident community feature so important? if important, describe what it is, else skip.}
Third, contrary to common belief, 
DNNs are \revision{not}
ubiquitous, especially in SS and WWW\techreport{,
due in part to limited data and computing resources availability, 
and to the lack of human interpretability of outputs}.
Lastly, in addition to reporting aggregate metrics,
authors often conduct fine-grained case studies on specific datapoints 
to study the limitations of their approach.  
Almost every CV paper contains case studies since images lend themselves to visualization.
Furthermore, NS papers often study specific high-impact features
to derive new scientific insights.

%\begin{figure}
%\centering
%\includegraphics[scale=0.55]{figures/funSurveyFacts}
%\caption{Notable Characteristics of ML Workflows by Domain.}
%\label{fig:funFact}
%\end{figure}

We use iteration trends and insights presented in Figure~\ref{fig:survey}
to guide our system design and empirical evaluation.

% common metrics?


%  ------ old version below -------
%\shit{Common ML folklore knowledge indicates that ML workflows are seldom ``perfect''
%on the first attempt and require significant iteration
%to improve accuracy~\cite{lin2013scaling,sumbaly2013big}.
%To confirm this, we surveyed papers
%from a variety of machine learning application areas to check for
%the presence of {\em workflow iterative actions}, involving some sort of
%user-instigated modification of one or more ML workflows presented in each paper.
%%We found that nearly every paper had some example of a {\em workflow action};
%%that is, a tweak to the data preparation, learning, or inference step(s) of a given workflow.
%Naturally, this survey has one major limitation ---
%authors often omit the exact number
%of iterations 
%\dorx{It's not just the number we're interested in. 
%We need to know what the iterations are.} 
%taken along the way to the reported findings.
%Nonetheless, it provides valuable insights into the kinds
%of ``knobs'' that are often used to tune ML workflows.}
%
%%While iterating on machine learning workflows is a widely adopted practice
%%in developing real-world applications~\cite{lin2013scaling, sumbaly2013big},
%%we are not aware of any evidence that 
%%quantitatively characterizes this iterative process.
%%\dorx{Rewrote the sentence above because I didn't find any reference to iteration in \cite{munson2012study}.}
%%To remedy this, we conducted a small scale survey of 
%%the applied ML literature across multiple fields
%%to catalog the frequency of various workflow modification actions.
%%Naturally, this survey has one major limitation ---
%%authors often omit reporting on a number
%%of iterations the taken to get to the reported findings.
%%Nevertheless, it provides valuable insights into the kinds
%%of ``knobs'' that are often used to tune ML workflows.
%
%\shit{\agpquote{We selected 5 application areas for machine learning, and one or more
%publication venues for each of them---Social Sciences (KDD), Natural Sciences (KDD, Nature), Computer Vision (KDD, CVPR), Natural Language Processing (KDD, ACL), and Web Mining (KDD) with 25, 37, 20, 37, and 12 papers
%from each area, respectively. The papers were all published in either 2015 or 2016.}{Maybe provide some details?}
%\agpquote{``Iteration actions'' present in the papers fell broadly into two categories:
%data preparation (DPR), or learning/inference (L/I).
%DPR actions include addition, deletion, or transformation of the raw data~\cite{kuhn2013data}, and L/I iteration actions
%include any tweak to the learning algorithm, including
%(but not limited to) adjustment of regularization or other hyperparameters,
% model selection, ablations of the core workflow, and other modifications for error analysis.}{You are just repeating 2.1.}
% \ \\
% \agp{Can we provide some examples of interesting insights? E.g. NLP requires more blah. Right now, feels like
% you cooked up numbers from thin air.}
%\frameme{Overall, we found that
%{\em nearly every paper exhibited some sort of iteration on at least one ML workflow}, with
%a roughly 50/50 split between adjustments to DPR and adjustments to L/I.}}
%\placeholder{We will release our survey's paper list, its associated code,
%and our detailed analysis of the results along with the rest of the \gs codebase upon this manuscript's
%acceptance for publication.}
%\smc{Placeholder sentence until we decide whether we want to put more detailed survey plots in appendex,
%techreport, or release with code.}
%
%\hidden{We manually classified each variant of the ML workflow described
%in each of these papers based on \dorx{rewrite the rest of this section from this point.} a transformation to either DPR or L/I, where DPR generally refers to the addition, deletion, or transformation of the training set data\cite{kuhn2013data} and L/I refers to any operation towards machine learning algorithm.
%% \dorx{Iterating on the DPR component involves ..., whereas iterating on L/I involves ... I don't know if you need this sentence if you're listing the actions in the next one.}
%Within
%DPR, we classified each variant into either 
%feature selection (select a subset of features), feature normalization (normalize independent variables of features into the range [0,1]), or feature transformation (apply a set of operators such as \{$+$, $-$, $*$\} on the original feature values\cite{sondhi2009feature}), and within L/I, we classified each variant into either
%a change of machine learning algorithm (i.e., switch the current ML model type, such as substituting SVM for logistic regression), 
%a change in tuning parameters (also known as model tuning which is adjusting the hyperparameters of the model training algorithms),
%or a change in model structure (e.g. adding L1/L2-regularization or adding an attention layer). 
%
%\topic{Quantitative Study Results} 
%To catalog the frequency of DPR and L/I, we judge each paper separately, where each variant within DPR and L/I was recorded. 
%The results are tabulated in Figure~\ref{fig:actionresult}(a) - (c), where the X axis is organized along different application areas, and the Y axis is the proportion of papers containing the corresponding ML workflow variant on the X.
%Figure~\ref{fig:actionresult}(a) is for the proportion of DPR and L/I in 5 application areas. Figure~\ref{fig:actionresult}(b) is for the proportion of the 3 primary DPR variants (feature selection, feature normalization and feature transformation) and Figure~\ref{fig:actionresult}(c) is for the proportion of the 3 primary L/I variants (ML algorithm change, model tuning and model structure change).
%% , where the X axis is organized along different application areas, and the Y axis is, the proportion of the number of papers in sampling papers containing the corresponding ML workflow variant on the X.
%
%
%Of all the papers we surveyed every single one of them contained some kind of iterative actions.
%As can be seen from the figure, variants of both DPR and L/I
%are often explored in applied machine learning papers;
%% specifically, more than 50\% of ML application papers displayed some variants on either DPR or L/I. 
%Similarly, we find that all three DPR variants,
%and all three L/I variants are common across all application areas.
%That said, there were some interesting special cases.
%For example, Figure~\ref{fig:actionresult}(a) shows that experts in Natural Sciences make more effort on Learning/Inference, which is different from experts in other application areas. This may because that experts in this application area are not quite familiar with ML. Therefore, when they try to optimize their ML workflow, they are not as confident with what is the right "general approach" and thus try different hyperparameters or just change their ML algorithm. 
%% By refering to Figure~\ref{fig:actionresult}(b), we notice that experts in Web Mining do more feature selection optimization than others. It is because that they 
%% Experts in Computer Vision make much more effort on feature transformation. It may be due to that a main problem in this area is how to interpret images and the problem convert to how to transform a image into better features when applying ML.
%% \dorx{break this into multiple sentences or condense. Also, you might want to give examples of feature transformations they do in CV because most readers would raise an eyebrow at the claim that a lot of feature transformation is done in CV.} 
%% Therefore, experts in this area use transformation processes to improve prediction accuracy. 
%Besides, we can find from Figure~\ref{fig:actionresult}(c) that experts in Natural Language Processing and Computer Vision have much more tendency to change model structure than others. It is because that experts in these areas use neural network to solve their problem frequently (more than 50\% of the sampling papers use neural network as one of the ML models) and thus they do more actions like add or remove a layer when adjusting the ML algorithm.}

% model structure change is the most frequent for experts in Natural Language Processing and Computer Vision when they tend to adjust their ML models, which 

% \dorx{Break into multiple sentences or condense. At this point I'm still puzzled by the result that CV people do a lot of feature transformations despite using NNs, which are supposed to reduce the need for feature engineering.}


% the tendency to pay more attention on transforming text data into appropriate data format in order to implement ML methods and improve prediction accuracy.







 % This may be caused by that experts in this application area have more tendency to make effort on how to build their ML model such as tuning the hyperparameters and changing the structure of model (shown in Figure~\ref{fig:actionresult}(c)).  For data preparation, they usually only use several sentences to explain how they select the features.


  % By referring to Figure~\ref{fig:actionresult}(b), it is shown that experts in Natural Language Processing make much more effort on feature transformation, which may be due to the tendency to pay more attention on transforming text data into appropriate data format in order to implement ML methods and improve prediction accuracy. 



  





% the variants in all application areas are on DPR and on L/I. 







% By referring to Figure~\ref{fig:actionresult}c), that condition is partly beacuse 




% \agp{plot has TOO small of a font. Needs to be much larger. It's Learning/Inference, 
% not Learning. "Detail in Blah" can be avoided. Just say "Data Preparation Breakdown", "Learning/Inference Breakdown" etc.}

% \agp{potentially delete everything below once gaps are filled in ==========}


% \todo{\dorxsubst{Stas}{Stats} work and need some comment}
% \dorx{What is an action in the context of this section?}
% As is mentioned above, ML workflows can be decomposed to data preparation and learning/inference. We regard these two components as two main actions in ML: Data Preparation and Learning. 
% \dorx{Two main categories of actions maybe. 
% They are not refinement actions themselves.}
% \dorxsubst{Data Preparation generally refers to}
% {Iterative refinements to the data preparation component may include} the addition, deletion, or transformation of the training \dorxout{set} data\cite{kuhn2013data}. 
% It contains feature selection, feature formats transformation, normalization etc. Learning contains actions of switching different types of model, modifying objective model structure, model tuning etc. 
% \dorx{Okay none of these terms mean much to someone who has little ML background. 
% Put them in the context of what has already been introduced.}

% Action information is what indicates the machine learning users' actions. 
% \dorxout{To refine the iteration,} we evaluate what experts in different research field tend to do in order to optimize their ML workflow by \dorxsubst{randomly selecting}{sampling} 120 papers from KDD 2016, ACL 2016 and Nature and extracting action information from them. According to the papers used, we divide the research field into 5 aspects: Social Sciences, Natural Sciences, Computer Vision, Natural Language Processing and Web Mining. The results are shown in Figure~\ref{fig:actionresult}.

% \dorx{What is the overall trend before you talk about individual subject areas.}
% \dorxsubst{According to}{As shown in} Figure~\ref{fig:actionresult}a), experts in Social Sciences, Computer Vision, Natural Language Processing and Web Mining make more effort on data preparation. However, Natural Sciences experts do more things on learning. For data preparation, Figure~\ref{fig:actionresult}b) shows that transforming feature formats is the most frequent action for experts in Computer Vision and Natural Language Processing and filter/select feature is the most frequent in other research field. For learning stage, Computer Vision and Natural Language Processing experts have a greater tendency to modify model structure, but experts in other research field make more effort on model tuning.
% \dorx{Okay can you say something about what contributes to this difference?}

% ML workflow iteration can be refined based on different tendency of different research field.


% \todo{add figures}
% We divided Learning/inference into two sub-category: Model Specification and Optimization. Any modification to the objective component of a machine learning model is a Model Specification action, such as switching the model, modifying objective model structure and model tuning. Optimization are actions that optimize the performance of the model on the basis of not changing the objective component of the model, such as adjusting batchsize of the neural network. Besides, changing the iteration number is also Optimization. 
% Result(figure) and comment?
% \todo{add .did add picture}
% \todo{outline}






==> overview-workflows.tex <==
%!TEX root=../dml.tex

A machine learning (ML)
workflow accomplishes a specific ML task,
 ranging from simple ones like classification or clustering,
 to complex ones like entity resolution or image captioning.
 The more complex tasks are often broken down into smaller subtasks;
 e.g., image captioning is broken down into 
 identifying objects or actions via classification,
 followed by generating sentences using a language model~\cite{karpathy2015deep}.
Within \name, we decompose ML workflows into three components:
\dataprep~(DPR), learning/inference (L/I), and postprocessing (PPR).
These three components are generic and 
adapt to a wide variety of supervised, semi-supervised, and unsupervised settings, as we will demonstrate in Section~\ref{sec:experiments}.
Let $\mathcal{R}$ be the raw input data for the ML workflow.

\topic{\Dataprep~(DPR)} During \textit{\dataprep}, $\mathcal{R}$ is transformed, 
through a series of operations, into some representation 
$\mathcal{D} \in \mathcal{X}$,
where $\mathcal{X}$ is the input for model training.
The transformation from $\mathcal{R}$ to $\mathcal{D}$ 
can involve a variety of operations, 
such as fine-grained feature definition from individual attributes (e.g., number of vowels in a word), 
joining in other data sources (e.g., user information into log data), 
parsing (e.g., a document to words), and 
aggregation (e.g., aggregating ad clicks).


\topic{Learning/Inference (L/I)}
During \textit{learning}, an algorithm is run on $\mathcal{D}$ 
to obtain a model $f: \mathcal{X} \rightarrow \mathcal{Y}$, 
such as a linear classifier, decision tree, or cluster centers,
where $\mathcal{Y}$ denotes the space of the target outputs for the ML task.
Then, during \textit{inference}%
\techreport{\footnote{We use the term as defined in the ML community;
this term is not to be confused with \textit{statistical inference}, 
which is concerned with estimating distributions based on data. 
}}%
,
this model $f$  is used to process new data from $\mathcal{X}$.
For example, in spam classification, $f$ decides whether a new email is spam;
in clustering, $f$ assigns a datapoint to a specific (set of) cluster(s);
in image captioning, $f$ generates a text caption for an image;
and in word embeddings, $f$ maps a string containing a word onto a vector.
\techreport{
We treat learning and inference as a unified component 
because 
data processed by the DPR component can either be used for learning,
or, in the case a model has already been learned, inference.
As shown in the examples above, this observation
is valid for both supervised and unsupervised learning.
}

\topic{Post-processing (PPR)} 
Finally, an ML workflow usually contains 
additional operations on the output model or inference results. 
This could include model evaluation, 
visualizations, 
or other application-specific activities. 
We refer to these operations as \textit{postprocessing}.


==> syntax.tex <==
%!TEX root = ../dml.tex

Statements in \lang either declare new \name objects
and/or specify the relationship between existing ones via \textit{linking expressions}. 
%\red{\{}Linking expressions in \lang always connect DCs to operators or vice versa, 
%never two DCs or operators. 
%Thus, the declarations in a \name program form \textit{a bipartite graph between DCs and operators}. \red{\}}
%\agp{Why is this important? So what?}
\techreport{Expressions are infixed to mimic natural language, e.g., \code{word has\_extractors (first\_letter, last\_letter)}. 
Both DCs and operators are referenced by their string identifier in \lang, 
as shown in the syntax specifications in~\Cref{fig:syntax} (in~\Cref{sec:grammar}). }%
The complete set of linking expressions, along with their usages and functions, 
\papertext{can be found in the extended technical report~\cite{dorx2017}.}%
\techreport{is listed in Table~\ref{tab:semantics} (in~\Cref{sec:grammar}).} 
With just a handful of object types and linking expressions, 
\lang supports a wide range of use cases encompassing supervised and unsupervised learning 
in multiple domains.
We demonstrate this with four distinct applications in Section~\ref{sec:experiments}.
%For example, the input DC to \code{as\_example} can be the cartesian product obtained using $\times$, and so does the DC following \code{on}.

%\noindent \dorx{The following is nuanced.}
%\smc{bump to techreport?}
%\dorx{can do.}

% on doesn't form a complete statement, as shown in the syntax
%\placeholder{As shown in~\Cref{fig:syntax}, 
%\code{on} is the only linking expression that does not form a complete statement on its own.
%It needs to be followed by \code{as\_examples} in order to explicitly name the output DC
%so that the output can be referenced elsewhere in the program.
%% without "on", an implicit synthesizer is declared, as mentioned in the previous section.
%The \code{on} clause can be omitted if the default Synthesizer
%is used to form an Example by wrapping each SU in the input DC,
%as done in Line 17 and 18 in~\Cref{fig:wfEx}a).} \smc{placeholder text will go to techreport}



==> vldbreffix.tex <==
\usepackage{textcase}

\makeatletter
\def\@sect#1#2#3#4#5#6[#7]#8{%
    \ifnum #2>\c@secnumdepth
        \let\@svsec\@empty
    \else
        \refstepcounter{#1}%
        \edef\@svsec{%
            \begingroup
                %\ifnum#2>2 \noexpand\rm \fi % changed to next 29 July 2002 gkmt
                        \ifnum#2>2 \noexpand#6 \fi
                \csname the#1\endcsname
            \endgroup
            \ifnum #2=1\relax .\fi
            \hskip 1em
        }%
    \fi
    \@tempskipa #5\relax
    \ifdim \@tempskipa>\z@
        \begingroup
            #6\relax
            \@hangfrom{\hskip #3\relax\@svsec}%
            \begingroup
                \interlinepenalty \@M
                \if@uchead
                    \MakeTextUppercase{#8}% HERE
                \else
                    #8%
                \fi
                \par
            \endgroup
        \endgroup
        \csname #1mark\endcsname{#7}%
        \vskip -12pt  %gkmt, 11 aug 99 and GM July 2000 (was -14) - numbered section head spacing
\addcontentsline{toc}{#1}{%
            \ifnum #2>\c@secnumdepth \else
                \protect\numberline{\csname the#1\endcsname}%
            \fi
            #7%
        }%
    \else
        \def\@svsechd{%
            #6%
            \hskip #3\relax
            \@svsec
            \if@uchead
                \uppercase{#8}%
            \else
                #8%
            \fi
            \csname #1mark\endcsname{#7}%
            \addcontentsline{toc}{#1}{%
                \ifnum #2>\c@secnumdepth \else
                    \protect\numberline{\csname the#1\endcsname}%
                \fi
                #7%
            }%
        }%
    \fi
    \@xsect{#5}\hskip 1pt
    \par
}
\makeatother


